Structure-Aware Parametric Representations for Time-Resolved Light Transport

Time-resolved illumination provides rich spatio-temporal information for applications such as accurate depth sensing or hidden geometry reconstruction, becoming a useful asset for prototyping and as input for data-driven approaches. However, time-resolved illumination measurements are high-dimensional and have a low signal-to-noise ratio, hampering their applicability in real scenarios. We propose a novel method to compactly represent time-resolved illumination using mixtures of exponentially-modified Gaussians that are robust to noise and preserve structural information. Our method yields representations two orders of magnitude smaller than discretized data, providing consistent results in applications such as hidden scene reconstruction and depth estimation, and quantitative improvements over previous approaches.

==> src/0_abstract.tex <==
% old version
% Being able to capture light in motion requires special equipment, but enables a wide variety of applications such as material classification and reconstruction of partially or fully hidden geometry. However, these transient imaging methods suffer from huge memory requirements and noisy measurements, slowing potential wide use of applications. We propose a novel method of signal compression and denoising based on Exponentially Modified Gaussian distributions, which resemble the behaviour of light propagation over time. This compact representation of the data is up to 100 times smaller, while also having denoising properties that improve reconstruction results of non-line of sight imaging.

Time-resolved illumination provides rich spatio-temporal information for applications such as accurate depth sensing or hidden geometry reconstruction. However, time-resolved illumination measurements are high dimensional and have low signal-to-noise ratio, hampering their applicability in real scenarios. We propose a novel method to compactly represent time-resolved illumination using mixtures of exponentially-modified Gaussians that are robust to noise and preserve structural information. Our method yields representations two orders of magnitude smaller than discretized data, and unlike previous approaches it provides consistent results in hidden scene reconstruction applications. 

==> src/0_aux_defines.tex <==
%!TEX root = EMGMM.tex
% \newcommand{\fref}[1]{Figure~\ref{#1}}
% \newcommand{\tref}[1]{Table~\ref{#1}}
% \newcommand{\eref}[1]{Equation~\ref{#1}}
% \newcommand{\cref}[1]{Chapter~\ref{#1}}
% \newcommand{\sref}[1]{Section~\ref{#1}}
% \newcommand{\aref}[1]{Annex~\ref{#1}}

% Commenting tools
\definecolor{red}{rgb}{0.8,0,0}
\definecolor{purered}{rgb}{1,0,0}
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{green}{rgb}{0.0,0.5,0}
\definecolor{blue}{rgb}{0,0,0.75}
\definecolor{darkblue}{rgb}{0,0,0.55}
\definecolor{orange}{rgb}{0.9,0.3,0.1}
\definecolor{purple}{rgb}{0.6,0.0,0.6}
\definecolor{cyan}{rgb}{0.0,0.7,0.7}
\definecolor{darkgray}{rgb}{0.4,0.4,0.4}
\definecolor{bronze}{rgb}{0.8, 0.5, 0.2}
\definecolor{dorange}{rgb}{0.75, 0.4, 0.0}
\definecolor{black}{rgb}{0.0,0.0,0.0}


% notes can be enabled/disabled by using one command or another
\newcommand{\note}[3][magenta]{\textcolor{#1}{(\textbf{\textit{#2}: #3})}}
% add notes per person (xcolor provides extra to choose from)
\newcommand{\diego}[1]{\note[red]{Diego}{#1}}
\newcommand{\droyo}[1]{\note[dorange]{Droyo}{#1}}
\newcommand{\question}[1]{\note[blue]{Q}{#1}}
\newcommand{\victor}[1]{\note[green]{Víctor}{#1}}

\newcommand{\todo}[1]{\textcolor{cyan}{#1}}
\newcommand{\new}[1]{\textcolor{red}{#1}}

\newcommand{\julioc}[1]{\textcolor{blue}{\emph{(\textbf{Julio:} #1)}}}
\newcommand{\juliotxt}[1]{\textcolor{blue}{\emph{\textbf{Julio:} #1}}}
\newcommand{\julio}[1]{{\leavevmode\color{blue}{#1}}}
\newcommand{\revise}[1]{{\leavevmode\color{purple}{#1}}}
\newcommand{\old}[1]{{\leavevmode\color{black}{#1}}}

% Usual terms
\newcommand*{\pmapping}[0]{\emph{photon mapping}}
\newcommand*{\Pmapping}[0]{\emph{Photon mapping}}
\newcommand*{\PMapping}[0]{\emph{Photon Mapping}}
\newcommand*{\pbeams}[0]{\emph{photon beams}}
\newcommand*{\Pbeams}[0]{\emph{Photon beams}}
\newcommand*{\PBeams}[0]{\emph{Photon Beams}}
\newcommand*{\Ptracing}[0]{\emph{Path tracing}}
\newcommand*{\VPTracing}[0]{\emph{Volumetric Path Tracing}}
\newcommand*{\PTracing}[0]{\emph{Path Tracing}}
\newcommand*{\ptracing}[0]{\emph{path tracing}}
\newcommand*{\Bptracing}[0]{\emph{Bidirectional path tracing}}
\newcommand*{\bptracing}[0]{\emph{bidirectional path tracing}}
\newcommand*{\Metropolis}[0]{\emph{Metropolis light transport}}
\newcommand*{\brdf}[0]{\emph{BRDF}}
\newcommand*{\ns}[0]{\mathrm{ns}}

% Usual math and physics terms

\newcommand{\Tr}{{T_r}}
\newcommand{\abs}{\mu_a} %absorption coefficient
\newcommand{\sca}{\mu_s} %scattering coefficient
\newcommand{\ext}{\mu_t} %extinction coefficient
\newcommand{\alb}{{_\Lambda}}
\newcommand{\scalb}{\alpha}
\newcommand{\crossscat}{\kappa_s}
\newcommand{\crossabs}{\kappa_a}
\newcommand*{\pf}[0]{\rho}
\newcommand*{\coefext}[0]{\sigma_t}
\newcommand*{\coefextx}[0]{\ext(x)}
\newcommand*{\coefabs}[0]{\sigma_a}
\newcommand*{\coefabsx}[0]{\abs(x)}
\newcommand*{\coefscat}[0]{\sigma_s}
\newcommand*{\coefscatx}[0]{\sca(x)}
\newcommand*{\mcoefext}[0]{$\coefext$}
\newcommand*{\mcoefextx}[0]{$\coefextx$}
\newcommand*{\mcoefabs}[0]{$\coefabs$}
\newcommand*{\mcoefabsx}[0]{$\coefabsx$}
\newcommand*{\mcoefscat}[0]{$\coefscat$}
\newcommand*{\mcoefscatx}[0]{$\coefscatx$}
\newcommand*{\phasefunction}[0]{p(x, \vec{\omega}^\prime, \vec{\omega})}
\newcommand*{\ior}[0]{\eta}
%Usual equation expressions
\newcommand{\diff}{\mathrm{d}}
\newcommand{\where}{,\quad \text{where} \quad}
%\newcommand{\where}{\mid}
\newcommand{\omegav}{\vec{\omega}}
\newcommand{\omegaout}{\omegav_o}
\newcommand{\omegain}{\omegav_i}
\newcommand{\momegain}{$\omegain$}
\newcommand{\ppwr}{\Phi}
\newcommand{\eqbreak}{\nonumber \\}
\newcommand{\x}{\ensuremath{\mathbf{x}}\xspace}
\newcommand{\y}{\ensuremath{\mathbf{y}}\xspace}
\newcommand{\z}{\ensuremath{\mathbf{z}}\xspace}
\newcommand{\rvec}{\vec{\ensuremath{\mathbf{r}}}\xspace}
\newcommand{\rlen}{\ensuremath{\mathrm{r}}\xspace}
\newcommand{\xpr}{\ensuremath{\mathbf{x}^\prime}\xspace}
\newcommand{\xm}{{\x}}
\newcommand{\xc}{{\x_r}}
\newcommand{\xb}{{\xm_b}}
\newcommand{\ym}{{\y}}
\newcommand{\zm}{{\z}}
\newcommand{\VRegion}{\ensuremath{\aleph}\xspace}
\newcommand{\xs}{\ensuremath{\x_{s}}\xspace}
\newcommand{\ys}{\ensuremath{\y_{\! s}}\xspace}
\newcommand{\xw}{\ensuremath{\hat{\x}}\xspace}
\newcommand{\yw}{\ensuremath{\hat{\y}}\xspace}
\newcommand{\mpar}{r}
\newcommand{\pkern}{\Omega}
\newcommand{\optpath}{\Pi}


% Paper specifics
\newcommand{\Enc}{\mathbf{E}} 	% Encoder function
\newcommand{\Dec}{\mathbf{D}} 	% Decoder function
\newcommand{\Trf}{g} 			% Transform function over data
\newcommand{\iTrf}{g^{-1}} 		% Inverse transform function over data
\newcommand{\Img}{\mathcal{H}}  % Transient image
\newcommand{\fts}{f_\Lref} 		% Feature vector of L
\newcommand{\Reals}{\mathbb{R}} % Real numbers
\newcommand{\tv}{t}
\newcommand{\Lref}{L} 			% Reference radiance
\newcommand{\Lij}{\Lref_{ij}}
\newcommand{\aLij}{{\hat{\Lref}}_{ij}}		
\newcommand{\Lijt}{\Lij(\tv)}
\newcommand{\aLijt}{\aLij(\tv)}
\newcommand{\Lnxn}{\langle\Lij\rangle}
\newcommand{\thrs}{\varepsilon}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\Church}{\emph{Altar}\xspace}
\newcommand{\Building}{\emph{Building}\xspace}
\newcommand{\Livingroom}{\emph{Living room}\xspace}
\newcommand{\House}{\emph{Balcony}\xspace}
\newcommand{\Kitchen}{\emph{Kitchen}\xspace}


==> src/1_introduction_related_work.tex <==
\begin{figure*}[!t]
	\centering
	\includegraphics[width=\linewidth]{figures/teaser_horizontal_fix_v3.pdf}
	%\includegraphics[width=1.0\columnwidth]{square_pattern}
	\caption{Application of our method to non-line-of-sight (NLOS) data for a real scene. Top: original captured signal. Bottom: adding noise simulating an exposure time 200 times shorter. The scene is then reconstructed following the work by Liu et al. \cite{liu2019non}. On the right, we show the results using the original captured signal and the compressed signals using the autoencoder network proposed by Liang et al. \cite{liang2020compression}, and our method.}
	\label{fig:nlos-reconstruction}
\end{figure*}
%
Transient imaging methods analyze time-resolved light transport at very high temporal resolution, with applications such as reconstruction of hidden geometry \cite{Lindell2019wave,liu2019non,Xin2019theory}, object detection through scattering media \cite{Heide2014}, or material classification \cite{su2016material}, with promising advances over the recent years \cite{jarabo2017recent}. Current capture methods combine ultra-fast lasers with sensors such as Single Photon Avalanche Diode (SPAD) arrays \cite{renna2020fast, nam2021low}, providing dense spatial scanning and picosecond temporal resolution that yield rich spatio-temporal information of the captured scene. 



% Newer setups such as Photonic Mixer Devices (PMD) \cite{Heide2013} are more accessible, but sacrifice temporal and spatial resolution. For these reasons, light transport simulation \cite{Jarabo2014} is also commonly used.
These capture setups, however, introduce several limitations. 
% However, despite recent advances, transient imaging methods are struggling for wider applications. Data, both captured and simulated, has two main limitations. 
First, analyzing the spatio-temporal structure of indirect illumination is fundamental in many transient imaging applications, but multiply scattered light can become too attenuated when reaching the sensor. In consequence, imaging applications may be subject to measurements with low signal-to-noise ratio (SNR), which can decrease their performance. 
%
%Meanwhile, noise can be introduced by capture devices (e.g. dark counts in SPADs), ambient illumination or variance in Monte Carlo simulation. 
%
Second, dense temporal and spatial resolutions of the measurement space result in high memory and bandwidth requirements (with datasets of tens or hundreds of gigabytes) \cite{marco2021NLOSvLTM}, which can become a bottleneck in light transport analysis and application design. 



In this work we provide a method for lightweight representations of time-resolved illumination with a three-fold benefit: the representation space is up-to two orders of magnitude smaller than source data and two times smaller than previous compression approaches, it is robust to noise, and it preserves structural information fundamental in transient imaging applications. We rely on mixtures of exponentially-modified Gaussian (EMG) distributions, and design an optimization procedure that accounts for spatial gradients to preserve structural information.



Several previous works propose alternative representations of time-resolved light pulses with different goals. Note that none of these methods is structure-aware, as they only use temporal information from single points in the scene.
%
Peters et al. \cite{Peters2015} use the Pisarenko and maximum entropy spectral estimates to reconstruct transient pulses and improve data quality by removing multipath interference in range imaging.
%
For these same purposes, Kadambi et al. \cite{Kadambi2013} recover per-pixel sparse time profiles expressed as a sequence of impulses.
%
Other works are based on linear inverse problems \cite{Heide2014diffuse} solved by numerical optimization, and frequency-domain reconstructions \cite{Lin2014} which introduce Fourier analysis to reduce systematic errors.
%
% Simpson et al. \cite{2005Intensity} propose an Amplitude Modulated Continuous Wave (AMCW) technique for Lidar systems to recover the light scattering function. 
%
Closer to our representation space, Wu et al. \cite{Wu2014} analyze direct and indirect illumination components by representing light pulses as a combination of one Gaussian and one exponentially-modified Gaussian.
%
Heide et al. \cite{Heide2014} recovers time-resolved illumination in turbid media from correlation-based sensors by sparsely encoding light with EMG distributions.
%


Directly related to our goal, Liang et al. \cite{liang2020compression} recently introduced feature-based compact representations of time-resolved illumination using deep encoder-decoder neural architectures. However, their approach is biased towards line-of-sight training data, and fails to preserve structural information that is fundamental in modern transient imaging applications. As shown in \fref{fig:nlos-reconstruction}, our method yields representations of transient illumination with higher quality and that preserve structural information, providing significantly better performance on hidden geometry reconstructions than feature-based methods, even with a higher compression ratio.

Inspired by previous works \cite{Wu2014,Heide2014}, we propose to use exponentially modified Gaussian (EMG) distributions to compactly represent time-resolved illumination. Consider a transient camera which adds a third temporal dimension $T$ for an image $I$ with size $W \times H$, i.e. $I[i, j, t] \in \mathbb{R}^{W \times H \times T}$. A time-resolved pixel $I_\textbf{p}[t] \in \mathbb{R}^{1 \times 1 \times T}$ at $\textbf{p} = \{i, j\}$ represents the accumulation of light paths with a timestamp $t$ traveling from the light sources to the sensor pixel $\textbf{p}$ after being scattered through the scene elements. Time-resolved illumination typically has the temporal shape of aggregated radiance pulses with exponential decay. This behavior stems from multi-bounce convolutions of the source illumination pulse with the scene geometry. 
%
EMG distributions model a Gaussian with a parameterized exponential decay, and therefore arise as a convenient function to model physical behavior of different illumination bounces in time \cite{Wu2014,Heide2014}. We therefore propose to represent the response of a pulsed source measured at an ultra-fast sensor pixel by aggregating EMG distributions in a mixture model. We extensively analyze our approach on simulated time-resolved datasets, \emph{DeepToF} \cite{MarcoSIGA2017DeepToF} (line-of-sight scenes) and \emph{Z-NLOS} \cite{galindo19-NLOSDataset} (non-line-of-sight or NLOS scenes), and finally demonstrate its effectiveness on NLOS reconstruction applications \cite{liu2019non} under captured data.

==> src/2_contribution.tex <==
\paragraph{Exponentially-modified Gaussians}
An exponentially-modified Gaussian (EMG) distribution is defined as
\begin{align}
\operatorname{EMG}(t; h, \mu, \sigma, \tau )=\frac{h\sigma}{\tau} \sqrt{\frac{\pi}{2}}\exp \left( \frac {1}{2} \left( \frac {\sigma}{\tau} \right)^2 - \frac {t-\mu}{\tau} \right) \nonumber \\
* \operatorname{erfc} \left( \frac {1}{\sqrt{2}}\  \left( \frac {\sigma}{\tau}  - \frac {t-\mu}{\sigma} \right) \right ),
\label{eq:EMG}
\end{align}
where $h$ controls the pulse amplitude, $\tau$ controls the exponential decay rate, and the mean $\mu$ and standard deviation $\sigma$ control the peak position and width of the Gaussian distribution. The complementary error function, $\text{erfc}(\cdot)$, is defined as
\begin{equation} \label{eq:ERFC}
\operatorname {erfc}(x)=
%1-\operatorname {erf}(x)=
{\frac  {2}{{\sqrt  {\pi }}}}\int _{x}^{\infty }e^{{-t^{2}}}\,dt.
\end{equation}
%
In our method we model the aggregation of multi-bounce light paths on a time-resolved single pixel $I_\textbf{p}[t]$ as an EMG mixture model ($\operatorname{EMGMM}$) with $K$ EMGs, denoted as $I_\textbf{p}^{\prime}[t]$,
\begin{align}
{I}_{\textbf{p}}[t] \approx {I}_{\textbf{p}}^{\prime}[t] &  = \operatorname{EMGMM}(t; \boldsymbol{h_{p}}, \boldsymbol{\mu_{p}}, \boldsymbol{\sigma_{p}}, \boldsymbol{\tau_{p}}, K)  \nonumber \\
% \label{eq:Ip} 
&= \sum _{k=1}^{K} \operatorname{EMG}(t; h_k, \mu_k, \sigma_k, \tau_k),
\label{eq:EMGMM}
\end{align}
where each $\boldsymbol{a}_p$ term represents a vector of $K$ EMG parameters $a_k$ with $k=1..K$ for the estimation of pixel $\textbf{p}$.



We formulate the estimation of a transient pixel $I_\textbf{p}[t] \approx I_\textbf{p}^\prime[t]$ as an optimization problem which attempts to compute the best EMGMM parameterization $\{\boldsymbol{h_p},\boldsymbol{\mu_p},\boldsymbol{\sigma_p},\boldsymbol{\tau_p}\}$ in order to minimize the pixel loss function $\mathcal{L}_p$:
%
\begin{align}
\mathop{\arg\min}\limits_{\boldsymbol{h_p},\boldsymbol{\mu_p},\boldsymbol{\sigma_p},\boldsymbol{\tau_p}} \mathcal{L}_p(I_\textbf{p},I_\textbf{p}^{\prime}),
\label{eq:single_pixel_optimization}
\end{align}
where $\mathcal{L}_p$ is lower when both time-resolved illumination distributions are more similar. Since we are working with EMG distributions, we define $\mathcal{L}_p$ based on the Kullback-Leibler Divergence (KLD) \cite{kullback1951information}, a statistical distance metric used to measure the difference of probability distributions. For a pixel $I_\textbf{p}$ and its reconstruction $I_\textbf{p}^{\prime}$, the KLD is defined as
%
\begin{align}
\displaystyle D_{\text{KL}}(I_\textbf{p}^{\prime} \parallel I_\textbf{p}) = \sum_{t\in T}I_\textbf{p}^{\prime}[t]\log \left({\frac {I_\textbf{p}^{\prime}[t]}{I_\textbf{p}[t]}}\right).
\end{align}
Note that KLD is asymmetric, and also produces low errors where $I_\textbf{p}^{\prime} \approx 0$ and high errors where $I_\textbf{p} \approx 0$. To avoid these extreme cases, we use its asymmetric property to finally construct our pixel loss function $\mathcal{L}_p$:
%
\begin{align}
  \mathcal{L}_p(I_\textbf{p},I_\textbf{p}^{\prime}) &= \displaystyle D_{\text{KL}}(I_\textbf{p}\parallel I_\textbf{p}^{\prime})+D_{\text{KL}}(I_\textbf{p}^{\prime}\parallel I_\textbf{p})
  \nonumber \\
%   &= \sum_{t\in {T}}I_\textbf{p}[t]\log \left({\frac {I_\textbf{p}[t]}{I_\textbf{p}^{\prime}[t]}}\right) + \sum_{t\in {T}}I_\textbf{p}^{\prime}[t]\log \left({\frac {I_\textbf{p}^{\prime}[t]}{I_\textbf{p}[t]}}\right) \nonumber \\
  &= \sum_{t\in {T}}(I_\textbf{p}[t]-I_\textbf{p}^{\prime}[t])(\log{(I_\textbf{p}[t])} - \log{(I_\textbf{p}^{\prime}[t])}).
  \label{eq:lossfunction}
\end{align}
%
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\columnwidth]{figures/emg-network.pdf}
	\caption{Left: EMGMM with $K$ EMG modules. Right: EMG substructure with four parameters and one input connected to the Probability Mass Function (PMF) node corresponding to \eref{eq:EMG}. To ensure $h, \sigma, \tau > 0$, an exponential function is applied. As $t \in [0, 1]$ is normalized, a $\text{sigmoid}$ function is applied to $\mu$.}
	\label{fig:model_structure}
\end{figure}
%
Given that $\mathcal{L}_p$ (\eref{eq:lossfunction}) and EMGs (Equations \ref{eq:EMG} and \ref{eq:ERFC}) are differentiable, we use Stochastic Gradient Descent to optimize for the best parameters in an EMG-based differentiable pipeline shown in \fref{fig:model_structure}. For an input time $t$, the pipeline should output the pixel intensity at that time $I_\textbf{p}^{\prime}[t]$.



Other loss functions such as the Mean Square Error (MSE) \cite{liang2020compression} tend to be biased towards large-valued regions in the temporal domain, which may lead the optimization to fall into local minima. Our KLD-based optimization reduces the error more uniformly across the entire temporal domain, shown in \tref{tab:optimization-order} when compared to the MSE-based approach.



For practical reasons, we pre-process the optimization input as follows: we first clip the temporal domain of each pixel $I_\textbf{p}[t]$ to $t\in[t_\text{start}, T]$, where $I_\textbf{p}[t_\text{start}]$ the first non-zero value. We then normalize the clipped temporal domain to $t \in [0, 1]$ subtracting $t_\text{start}$ and dividing by the resulting length $T' = T - t_\text{start}$. The EMGMM (\eref{eq:EMGMM}) is therefore evaluated in a reparameterized time interval $t\in [0, 1]$, where the reference pixel $I_\textbf{p}[t]$ does not have leading zeroes. We store $t_{start}$ and $T'$ along with the $4K$ EMGMM parameters $\boldsymbol{h_p},\boldsymbol{\mu_p},\boldsymbol{\sigma_p},\boldsymbol{\tau_p}$, and revert the clipping and normalization to compute the loss (\eref{eq:lossfunction}), resulting in a final compression factor of ${T}/{(4K+2)}$.

\paragraph{Reconstructing a transient image} \eref{eq:single_pixel_optimization} defines the optimization scheme to represent a single pixel $I_\textbf{p}[t]$, with $\textbf{p}=\{i,j\}$ using a EMGMM. For a full transient image $\equiv I[i, j, t]$, neighbouring pixels usually present significant spatio-temporal structure. In the following we propose an optimization methodology to use spatio-temporal information to improve the representation of the pixels in a transient image with a two-fold benefit. First, reduction of noise in low SNR areas by leveraging noisy information from nearby pixels. Second, preserving the spatial structure of the signal by accounting for spatial gradient. In particular we use the $N \times N$ neighbourhood around each pixel $\textbf{p}$, noted as $\mathcal{W}(\textbf{p}, N) \equiv \mathcal{W}$ and defined as all pixels $\textbf{p}^{\prime}$ where $\Vert \textbf{p}^{\prime} - \textbf{p} \Vert_\infty < N/2$. We introduce a spatial gradient loss term $\mathcal{L}_g$ that fosters consistency between neighbouring pixels, reducing the influence of per-pixel noise:
%
\begin{align}
  \mathcal{L}_g(I_\mathcal{W},I_\mathcal{W}^{\prime}) = \sum_{t \in T} & \Big( \parallel{G_\text{up}(I_\mathcal{W}, t) - G_\text{up}(I_\mathcal{W}^{\prime}, t)}\parallel_2 \nonumber \\
  &+ \parallel{G_\text{down}(I_\mathcal{W}, t) - G_\text{down}(I_\mathcal{W}^{\prime}, t)}\parallel_2 \nonumber \\
  &+ \parallel{G_\text{left}(I_\mathcal{W}, t) - G_\text{left}(I_\mathcal{W}^{\prime}, t)}\parallel_2 \nonumber \\
  &+ \parallel{G_\text{right}(I_\mathcal{W}, t) - G_\text{right}(I_\mathcal{W}^{\prime}, t)}\parallel_2 \Big).
  \label{eq:LossG}
\end{align}
%
Each gradient $G$ is defined for a neighbourhood $\mathcal{W}$ where each element is computed using its immediate neighbours as
%
\begin{equation}
	\left\{
	\begin{aligned}
 	&G_\text{up}(I_\mathcal{W}, t) &= I[i, j - 1, t] - I[i, j, t] \\
  	&G_\text{down}(I_\mathcal{W}, t) &= I[i, j + 1, t] - I[i, j, t] \\
  	&G_\text{left}(I_\mathcal{W}, t) &= I[i - 1, j, t] - I[i, j, t] \\
 	&G_\text{right}(I_\mathcal{W}, t) &= I[i + 1, j, t] - I[i, j, t]
	\end{aligned}
	\right.
	, \, \textbf{p} = \{i, j\} \in \mathcal{W},
	\label{eq:gradient_loss}
\end{equation}
adding zero-padding on the image to satisfy the calculation for edge pixels. The final optimization problem is
\begin{align}
\mathop{\arg\min}\limits_{\boldsymbol{h}_\mathcal{W},\boldsymbol{\mu}_\mathcal{W},\boldsymbol{\sigma}_\mathcal{W},\boldsymbol{\tau}_\mathcal{W}}
\mathcal{L}_g(I_\mathcal{W},I_\mathcal{W}^{\prime}) +
\sum_{\textbf{p} \in W}
\mathcal{L}_p(I_\textbf{p},I_\textbf{p}^{\prime}),
\label{eq:final_optimization_problem}
\end{align}
%
reconstructing $N \times N$ pixels in the image simultaneously. The resulting optimization accounts for multiple EMGMMs as in \fref{fig:model_structure} for each pixel in the neighbourhood, calculating the gradient afterwards. Also, the data needs to be pre-processed as explained previously. The value of $t_\text{start}$ is obtained as the minimum for all pixels $\textbf{p} \in \mathcal{W}$ based on the first pixel that receives a photon. The compression ratio for the whole neighbourhood is $(N^2 \cdot T) / (N^2\cdot 4K + 2)$.
%
\begin{table}[tb]
\caption{KLD loss $\mathcal{L}_I = \sum_\textbf{p} \mathcal{L}_{p}(I_\textbf{p}, I'_\textbf{p})$ in a region of the \emph{Staircase} NLOS scene \cite{galindo19-NLOSDataset} with $K=64$ for pixel-independent ($\mathcal{L}_{p}$), and \emph{Sliding} and \emph{Random} structure-aware fitting ($\mathcal{L}_{p} + \mathcal{L}_g$). The \emph{Random} fitting is also tested with a MSE-based optimization.}
\label{tab:optimization-order}
\centering
\begin{tabular}{l|r|r|r|r|}
\cline{2-5}
 & \multicolumn{3}{c|}{\textbf{KLD loss}} & \multicolumn{1}{c|}{\textbf{MSE loss}} \\ \cline{2-5} 
 & \multicolumn{1}{c|}{$\mathcal{L}_p$} & \textbf{\begin{tabular}[c]{@{}c@{}}$\mathcal{L}_p + \mathcal{L}_g$\\[-4pt] \emph{Sliding}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\mathcal{L}_p + \mathcal{L}_g$\\[-4pt] \emph{Random}\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}$\mathcal{L}_p + \mathcal{L}_g$\\[-4pt] \emph{Random}\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{$\mathcal{L}_I$} & $0.012$ & $0.010$ & $\mathbf{0.008}$ & $0.010$ \\ \hline
% \multicolumn{1}{|l|}{PSNR $\uparrow$} & 133.6 & 134.9 & \textbf{135.9} & 135.5 \\ \hline
\end{tabular}
\end{table}



\paragraph{Initialization}
Since our optimization is based on a Stochastic Gradient Descent, it is crucial to provide a good initialization to avoid converging to bad local minima. Light transport in real-world scenes decays exponentially: short, high-energy paths arrive early and have higher temporal frequency, while lower-energy multiply-scattered paths with longer optical are smooth and arrive later in time. We use these observations to estimate a convenient initial values for the peak $\mu$, width $\sigma$ and decay rate $\tau$ of each of the $K$ EMG modeled pulses. Note that the amplitude $h$ is just a scale factor, so we arbitrarily initialize it as $h=1$.

For each parameter, we initialize values $v_i$ in log-space, which provides a 5-10\% error improvement with respect to linear-space initialization for a similar number of epochs. We uniformly sample $\xi_i \in [\log(v_\text{min}),\log({v_\text{max}})]$ and then convert to linear range as $v_i = \exp(\xi_i)$. First, we sample $K$ values for $\mu$ and $\sqrt{K}$ values for $\sigma$ and $\tau$, of which we generate all possible $K$ combinations. The first bounces with smaller $\mu$ are narrower, so they are assigned the smaller $\sigma$ and $\tau$ values. This is done in order for each of the $K$ values of $\mu$ and $(\sigma, \tau$) pairs. Under this initialization, illumination pulses centered at later timestamps $\mu$ will have a wider support $\sigma$ and a slower decay $\tau$.

To reconstruct an image $I[i, j, t] \in \mathbb{R}^{W \times H \times T}$ the order for which we optimize the pixels is important when using spatial consistency as in \eref{eq:final_optimization_problem}. A first approach would be to slide through the $N \times N$ image pixels while optimizing each pixel neighborhood. This can produce square artifacts, so we use a \emph{Random} sampling of the image and optimize multiple neighbourhoods until every pixel has converged. Our quantitative analysis shown of \tref{tab:optimization-order} shows that while the \emph{Sliding} approach provides better results than independently fitting each pixel, the \emph{Random} approach provides the best results.

%\begin{table}[]
%\caption{Different initialization results, showing the resulting loss after convergence (around 500 to 700 epochs)}
%\label{tab:initialization}
%\begin{tabular}{l|cccccc}
% & \multicolumn{3}{c|}{\textbf{Linear-space sampling}} & \multicolumn{3}{c}{\textbf{Log-space sampling}} \\ \hline
%$\mathcal{L}_p$ & \multicolumn{3}{r|}{x.xx} & %\multicolumn{3}{r}{\textbf{x.xx}} \\
%\end{tabular}
%\end{table}

% Initialization is one of the main factor that influence the behaviour of convergence when using Stochastic Gradient Desent algorithm. We proposed a heuristic initialization method based on the following observation on light transport: As the light travels through the scene, it bounces back and forth multiple times between objects with different materials and at different positions, the energy decay exponentially. so the time profile of a pixel composed by multiple impulse response shows that: high frequency components which caused by direct reflection with less travel distance has high intensity show up in early time in time profile, as time goes, components show up in later time has lower and lower frequency due to interreflection or subsurface scattering which has longer travel distance.

%The characteristics of time profile illustrate above can be modeled by tuning the parameters of each EMG components in the mixture model. There are 3 parameters in EMG (\eref{eq:EMG}) that control the shape and position: $\mu$ the mean of Gaussian, control the position of the peak; $\sigma$ the standard deviation of Gaussian, control the sharpness, model higher frequency with smaller value; $\tau$ the exponent relaxation time, control the skewness, model higher exponentailly decaying speed with smaller value. The final mean, variance, skewness of EMG distribution are as follow:

%\begin{align}
%Mean &: \mu + \tau \label{eq:EMG_mean}\\
%Variance &: \sigma ^{2}+\tau ^{2} \label{eq:EMG_variance}\\
%Skewness &: {\frac  {2\tau ^{3}}{\sigma ^{3}}}\left(1+{\frac  {\tau ^{2}}{\sigma ^{2}}}\right)^{{-3/2}} \label{eq:EMG_skewness}
%\end{align}

%\textbf{Sampling on \emph{log space}}
%\quad We sampling $n$ value for each parameter in its given range $[r_{p_{min}},r_{p_{max}}]$ by following step: 1) transform the range to the log domain $[\log({r_{p_{min}}}),\log({r_{p_{max}}})]$; 2) sampling $n$ values evenly in the log range, result in $[v_1,v_2,...,v_n]$; 3) apply it as the power of $e$, result in $[e^{v_1},e^{v_2},...,e^{v_n}]$.


% For an EMG Mixture Model, There are $K$ values need to be initialized for each parameter. We proposed 3 different combinations to generate initial value for $\mu$, $\sigma$ and $\tau$ (\fref{fig:init_method}):

% As for the initial value of $h$(\emph{amplitude}), its just a scale factor in EMG, so we set all of them to be 1.
% We did a comparison between these 3 initialization mehtod in Section 5.


==> src/3_results.tex <==
\paragraph{Results}
%
\begin{table}[tb]
\caption{KLD loss $\mathcal{L}_I = \sum_\textbf{p} \mathcal{L}_{p}(I_\textbf{p}, I'_\textbf{p})$ in the \emph{Bathroom} LOS scene \cite{MarcoSIGA2017DeepToF}, comparing each compressed image $I'$ with respect to the original image $I$ for different numbers $K$ of EMGs.}
\label{tab:compare_k}
\centering
\begin{tabular}{l|r|cccc|}
\cline{2-6}
 & \multirow{2}{*}{\textbf{Liang et al. }} & \multicolumn{4}{c|}{\textbf{Ours}} \\ \cline{3-6} 
 &  & \multicolumn{1}{c|}{\textbf{K=4}} & \multicolumn{1}{c|}{\textbf{K=16}} & \multicolumn{1}{c|}{\textbf{K=64}} & \textbf{K=144} \\ \hline
\multicolumn{1}{|l|}{$\mathcal{L}_I$} & $0.100$ & \multicolumn{1}{r|}{$0.020$} & \multicolumn{1}{r|}{$0.013$} & \multicolumn{1}{r|}{$0.011$} & \multicolumn{1}{r|}{$0.008$} \\ \hline
% \multicolumn{1}{|l|}{PSNR $\uparrow$} & 73.1 & \multicolumn{1}{r|}{78.9} & \multicolumn{1}{r|}{79.6} & \multicolumn{1}{r|}{82.5} & \multicolumn{1}{r|}{91.9} \\ \hline
\end{tabular}
\end{table}
%

We compare our work with the 3D convolutional autoencoder network recently proposed by Liang et al. \cite{liang2020compression}, designed for the same purpose. \fref{fig:nlos-reconstruction} shows an example with a real world NLOS imaging application, where the capture setups produce noisier measurements when compared to simulated data. Our work provides a higher quality representation of both the signal and hidden geometry reconstruction, while also improving on the robustness to noise. The compression ratio is also higher, $\frac{T}{(4\cdot K+2)} \approx {42}$ for the chosen $K$ value, while the autoencoder network by Liang et al. has a lower ratio of 32. The number of components $K$ introduces a trade-off between the representation efficiency and quality. \tref{tab:compare_k} shows a comparison of different $K$ values for the \emph{Bathroom} \cite{MarcoSIGA2017DeepToF} dataset. A small value of $K$ is enough to represent the signal with minimal error, surpassing deep-learning based methods even with only $K=4$ EMGs per pixel. \fref{fig:compare_decomp_k16} shows a comparison of scene \emph{Church} \cite{MarcoSIGA2017DeepToF} with $K=16$ EMGs per pixel, resulting in approximately 62 times less parameters than the original signal. This almost doubles the compression ratio of the autoencoder network by Liang et al., and produces more accurate representations. \fref{fig:compare_decomp_k64_5x5} displays another example that shows the importance of the $5\times{5}$ window with spatial gradient constraints, as it greatly improves the spatial and temporal consistency of the represented signal.

\begin{figure}[tb]
	\centering
	\includegraphics[width=\columnwidth]{figures/compare_decomp_k16_redrawnv3.pdf}
	\caption{Our representation of the signal in the \emph{Church} scene \cite{MarcoSIGA2017DeepToF}. The last row shows the time profile $I_\textbf{p}[t]$ for the pixel $\textbf{p}$ marked with a cross. The vertical dotted lines correspond to four different time instants $t$ for the images $I[i, j, t]$ above.}
	\label{fig:compare_decomp_k16}
\end{figure}

\begin{figure}[tb]
	\centering
	\includegraphics[width=\columnwidth]{figures/compare_decomp_k64_5x5_redrawnv3.pdf}
	\caption{Signal representation of a 10x10 region of \emph{Staircase} \cite{galindo19-NLOSDataset} scene, similar to \fref{fig:compare_decomp_k16}. Adding a 5x5 window with gradient constraints (fourth columns, red) produces much better results than independently fitting each pixel (third columns, green).}
	\label{fig:compare_decomp_k64_5x5}
\end{figure}

==> src/4_conclusion_future_work.tex <==
In conclusion, we presented a method to efficiently represent time-resolved light transport data based on exponentially modified Gaussians, significantly reducing the amount of coefficients required to represent time-resolved transport. Our optimization loss based on first-order spatial differences preserves spatial structure and reduces noise, which are fundamental aspects in transient imaging applications. We demonstrated the benefits of our method in both LOS and NLOS scenarios, overcoming previous approaches targeted to transient light transport compression.
%
Relating the EMG components of our representation to higher-order illumination bounces may help to increase quality of scene understanding applications such as multipath interference correction in depth imaging or hidden scene reconstruction. Additionally, analysis of the frequency components of our EMG-based representation could be exploited in wave-based NLOS imaging algorithms \cite{Lindell2019wave,liu2019non} to improve their computational efficiency.
